Numerical study of the microscopic structure of jammed systems: from inferring their dynamics to finite size scaling

In this thesis I present most of the results obtained during my PhD, where I worked on different subjects regarding jamming in systems of frictionless spheres. In particular, I focused on microscopic properties of jammed packings, such as the distribution of contact forces and interparticle gaps, as well as the single particle dynamics that occur near the jamming point. Several of these results have already been presented in Refs. [1,2], but here I include a more detailed analysis of some of them. Besides, all the results of the second chapter are new, even if related to such works.

==> Chapters/conclusions.tex <==
\chapter{Conclusions and future work}\label{chp:conclusions}


